CFA: Constraint-based Finetuning Approach for Generalized Few-Shot Object Detection

Few-shot object detection (FSOD) seeks to detect novel categories with limited data by leveraging prior knowledge from abundant base data. Generalized few-shot object detection (G-FSOD) aims to tackle FSOD without forgetting previously seen base classes and, thus, accounts for a more realistic scenario, where both classes are encountered during test time. While current FSOD methods suffer from catastrophic forgetting, G-FSOD addresses this limitation yet exhibits a performance drop on novel tasks compared to the state-of-the-art FSOD. In this work, we propose a constraint-based finetuning approach (CFA) to alleviate catastrophic forgetting, while achieving competitive results on the novel task without increasing the model capacity. CFA adapts a continual learning method, namely Average Gradient Episodic Memory (A-GEM) to G-FSOD. Specifically, more constraints on the gradient search strategy are imposed from which a new gradient update rule is derived, allowing for better knowledge exchange between base and novel classes. To evaluate our method, we conduct extensive experiments on MS-COCO and PASCAL-VOC datasets. Our method outperforms current FSOD and G-FSOD approaches on the novel task with minor degeneration on the base task. Moreover, CFA is orthogonal to FSOD approaches and operates as a plug-and-play module without increasing the model capacity or inference time.

==> figures/boxplot.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}
\begin{axis}[%
width=0.9\textwidth,
height=2.3in,
%at={(0in,0in)},
scale only axis,
xticklabel style = {font=\small},
ymin=24,
ymax=33,
xlabel style={font=\color{white!15!black}, at={(axis description cs:0.5,-0.06)}, anchor=north},
%xlabel={\small overall AP},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\small \color{black}},
every y tick/.append style={black},
%every minor tick,
yticklabel style={%
	/pgf/number format/.cd,
	fixed,
	fixed zerofill,
	precision=3,
},
ytick={24,25,26,27,28,29,30,31,32,33},
yticklabels = {{},{25},{26},{27},{28},{29},{30}, {31}, {32}, {33}},
xmin=0,
xmax=18,
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18},
xticklabels = {{},{},{},{5-shot},{},{},{},{},{},{10-shot},{},{},{},{},{},{30-shot},{},{},{}},
ylabel style={font=\color{black}, at={(axis description cs:-0.06,0.5)}, anchor=south},
ylabel={\small \textcolor{black}{overall AP}},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
%xmajorgrids,
%ymajorgrids,
legend pos = north west,
legend style={legend cell align=left, align=left, draw=black, {nodes={scale=0.70}}},
boxplot/draw direction=y
]

\addplot+ [boxplot prepared={draw position=1,
lower whisker=25, lower quartile=26,
median=27, upper quartile=28, box extend=0.5,
upper whisker=29},
] coordinates {};
\addplot+ [boxplot prepared={draw position=2,
lower whisker=25, lower quartile=26,
median=27, upper quartile=28, box extend=0.5,
upper whisker=29},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 3,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {30.1\\29.2\\ 29.3\\ 29.1\\ 28.7\\ 28.2\\ 29.1\\ 28.6\\ 29.3\\ 29.0\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 4,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {29.7\\29.6\\ 29.7\\ 29.1\\ 29.2\\ 28.6\\ 29.5\\ 29.1\\ 29.5\\ 29.3\\};
\addplot+ [boxplot prepared={draw position=5,
lower whisker=25, lower quartile=26,
median=27, upper quartile=28, box extend=0.5,
upper whisker=29},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 6,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {30.1\\28.6\\ 28.3\\ 28.4\\ 28.2\\ 28.3\\ 27.8\\ 28.5\\ 29.5\\ 29.3\\};

\addplot+ [boxplot prepared={draw position=7,
lower whisker=25, lower quartile=26,
median=27, upper quartile=28, box extend=0.5,
upper whisker=29},
] coordinates {};
\addplot+ [boxplot prepared={draw position=8,
lower whisker=25, lower quartile=26,
median=27, upper quartile=28, box extend=0.5,
upper whisker=29},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 9,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {30.8\\29.8\\ 30.0\\ 29.8\\ 29.6\\ 29.4\\ 30.1\\ 29.3\\ 30.3\\ 29.8\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 10,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {30.3\\30.4\\ 30.4\\ 30.3\\ 30.0\\ 29.7\\ 30.4\\ 30.0\\ 30.5\\ 30.4\\};
\addplot+ [boxplot prepared={draw position=11,
lower whisker=25, lower quartile=26,
median=27, upper quartile=28, box extend=0.5,
upper whisker=29},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 12,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {31.4\\30.3\\ 30.4\\ 30.0\\ 30.4\\ 29.8\\ 30.3\\ 29.9\\ 30.1\\ 30.4\\};
\addplot+ [boxplot prepared={draw position=13,
lower whisker=25, lower quartile=26,
median=27, upper quartile=28, box extend=0.5,
upper whisker=29},
] coordinates {};
\addplot+ [boxplot prepared={draw position=14,
lower whisker=25, lower quartile=26,
median=27, upper quartile=28, box extend=0.5,
upper whisker=29},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 15,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
   ] table [row sep=\\, y index = 0] {31.9\\30.7\\ 30.7\\ 30.7\\ 30.6\\ 30.5\\ 30.8\\ 30.9\\ 30.9\\ 30.5\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 16,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
   ] table [row sep=\\, y index = 0] {31.7\\31.1\\ 31.2\\ 31.0\\ 31.0\\ 31.0\\ 31.1\\ 31.2\\ 31.2\\ 30.8\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 17,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
   ] table [row sep=\\, y index = 0] {31.9\\30.7\\ 30.7\\ 30.7\\ 30.6\\ 30.5\\ 30.8\\ 30.9\\ 30.9\\ 30.5\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 18,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
   ] table [row sep=\\, y index = 0] {32.0\\31.9\\ 31.5\\ 31.8\\ 31.5\\ 31.5\\ 31.7\\ 31.9\\ 31.9\\ 31.5\\};
   
\end{axis}

%\node[anchor=east,text width=2.4cm,align=left,fill=white,draw=black!80,line width=0.1mm,font=\fontsize{12}{0}\selectfont] at (legendPos) {\ref{lab:patch} \large Patch \\ \vspace{1mm} \ref{lab:whole} \large Whole \\ \vspace{1mm} \ref{lab:wavelet} \large Wavelet};

\end{tikzpicture}%
\end{figure*}

==> figures/boxplot_old.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}
\begin{axis}[%
width=0.9\textwidth,
height=2.3in,
%at={(0in,0in)},
scale only axis,
xticklabel style = {font=\small},
ymin=0,
ymax=44,
xlabel style={font=\color{white!15!black}, at={(axis description cs:0.5,-0.06)}, anchor=north},
%xlabel={\small overall AP},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\small \color{black}},
every y tick/.append style={black},
%every minor tick,
yticklabel style={%
	/pgf/number format/.cd,
	fixed,
	fixed zerofill,
	precision=3,
},
ytick={0,5,10,15,20,25,30, 35, 40, 45},
yticklabels = {{},{5},{10},{15},{20},{25},{30}, {35}, {40}, {45}},
xmin=0,
xmax=18,
xtick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18},
xticklabels = {{},{},{},{5-shot},{},{},{},{},{},{10-shot},{},{},{},{},{},{30-shot},{},{},{}},
ylabel style={font=\color{black}, at={(axis description cs:-0.06,0.5)}, anchor=south},
ylabel={\small \textcolor{black}{overall AP}},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
%xmajorgrids,
%ymajorgrids,
legend pos = north west,
legend style={legend cell align=left, align=left, draw=black, {nodes={scale=0.70}}},
boxplot/draw direction=y
]

\addplot+ [draw= red, fill=red, boxplot prepared={draw position=1,
lower whisker=2.5, lower quartile=4,
median=8.5, upper quartile=12,
upper whisker=15},
] coordinates {};
\addplot+ [boxplot prepared={draw position=2,
lower whisker=2.5, lower quartile=4,
median=8.5, upper quartile=12,
upper whisker=15},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 3,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {30.1\\29.2\\ 29.3\\ 29.1\\ 28.7\\ 28.2\\ 29.1\\ 28.6\\ 29.3\\ 29.0\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 4,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {29.7\\29.6\\ 29.7\\ 29.1\\ 29.2\\ 28.6\\ 29.5\\ 29.1\\ 29.5\\ 29.3\\};
\addplot+ [boxplot prepared={draw position=5,
lower whisker=2.5, lower quartile=4,
median=8.5, upper quartile=12,
upper whisker=15},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 6,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {30.1\\28.6\\ 28.3\\ 28.4\\ 28.2\\ 28.3\\ 27.8\\ 28.5\\ 29.5\\ 29.3\\};

\addplot+ [boxplot prepared={draw position=7,
lower whisker=2.5, lower quartile=4,
median=8.5, upper quartile=12,
upper whisker=15},
] coordinates {};
\addplot+ [boxplot prepared={draw position=8,
lower whisker=2.5, lower quartile=4,
median=8.5, upper quartile=12,
upper whisker=15},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 9,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {30.8\\29.8\\ 30.0\\ 29.8\\ 29.6\\ 29.4\\ 30.1\\ 29.3\\ 30.3\\ 29.8\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 10,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {30.3\\30.4\\ 30.4\\ 30.3\\ 30.0\\ 29.7\\ 30.4\\ 30.0\\ 30.5\\ 30.4\\};
\addplot+ [boxplot prepared={draw position=11,
lower whisker=2.5, lower quartile=4,
median=8.5, upper quartile=12,
upper whisker=15},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 12,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
] table [row sep=\\, y index = 0] {31.4\\30.3\\ 30.4\\ 30.0\\ 30.4\\ 29.8\\ 30.3\\ 29.9\\ 30.1\\ 30.4\\};
\addplot+ [boxplot prepared={draw position=13,
lower whisker=2.5, lower quartile=4,
median=8.5, upper quartile=12,
upper whisker=15},
] coordinates {};
\addplot+ [boxplot prepared={draw position=14,
lower whisker=2.5, lower quartile=4,
median=8.5, upper quartile=12,
upper whisker=15},
] coordinates {};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 15,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
   ] table [row sep=\\, y index = 0] {31.9\\30.7\\ 30.7\\ 30.7\\ 30.6\\ 30.5\\ 30.8\\ 30.9\\ 30.9\\ 30.5\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 16,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
   ] table [row sep=\\, y index = 0] {31.7\\31.1\\ 31.2\\ 31.0\\ 31.0\\ 31.0\\ 31.1\\ 31.2\\ 31.2\\ 30.8\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 17,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
   ] table [row sep=\\, y index = 0] {31.9\\30.7\\ 30.7\\ 30.7\\ 30.6\\ 30.5\\ 30.8\\ 30.9\\ 30.9\\ 30.5\\};
\addplot+[%
    mark = *, %
    fill=red,
    draw=red,
    opacity=0.5,
    boxplot = {%
    draw position = 18,
     average = auto,%
     every average/.style={/tikz/mark=diamond*},
     every median/.style={/tikz/draw=black},
     box extend=0.5
    }, %
   ] table [row sep=\\, y index = 0] {32.0\\31.9\\ 31.5\\ 31.8\\ 31.5\\ 31.5\\ 31.7\\ 31.9\\ 31.9\\ 31.5\\};
   
\end{axis}

%\node[anchor=east,text width=2.4cm,align=left,fill=white,draw=black!80,line width=0.1mm,font=\fontsize{12}{0}\selectfont] at (legendPos) {\ref{lab:patch} \large Patch \\ \vspace{1mm} \ref{lab:whole} \large Whole \\ \vspace{1mm} \ref{lab:wavelet} \large Wavelet};

\end{tikzpicture}%
\end{figure*}

==> figures/figure_training_settings.tex <==
\begin{figure*}[h]
 \centering
 \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.95\linewidth,  height=0.45\linewidth]{figures/fsod_finetuning.pdf}
    \caption{Finetuning stage in FSOD setting.}
    \label{fig:FSOD}
 \end{subfigure}
 \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.95\linewidth,  height=0.45\linewidth]{figures/gfsod_finetuning.pdf}
    \caption{Finetuning stage in G-FSOD setting.}
    \label{fig:GFSOD}
 \end{subfigure}
  \caption{Training Stage- Finetuning Stage}%
  \label{fig:training_settings}%
\end{figure*}

==> tables/ablation_agem_old.tex <==
\begin{table}[] \centering
	\setlength{\tabcolsep}{1.7mm}
	\scalebox{0.86}
	{\begin{tabular}{c|ccc|ccc}
			%\hline
			\toprule[1.1pt]
			\multicolumn{1}{c|}{}    &\multicolumn{3}{c|}{} &\multicolumn{3}{c}{}\\
			\multicolumn{1}{c|}{\multirow{-2}{*}{Model}}  & \multicolumn{1}{c}{\multirow{-2}{*}{AP}} & \multicolumn{1}{c}{\multirow{-2}{*}{bAP}}  &  \multicolumn{1}{c|}{\multirow{-2}{*}{nAP}} & \multicolumn{1}{c}{\multirow{-2}{*}{AR}} & \multicolumn{1}{c}{\multirow{-2}{*}{bAR}}  &  \multicolumn{1}{c}{\multirow{-2}{*}{nAR}}                 \\
			\midrule[0.9pt]
			  A-GEM w/ fc & 30.1 & 36.8 & 10.1 & 46.0 & 54.4 & 20.7\\
			  \rowcolor[HTML]{EFEFEF}
			  CFA w/ fc & 30.8 & \textbf{37.6} & 10.5 & 43.7 & 50.4 & 23.6 \\\hline
			  A-GEM w/ cos & 28.2 & 34.5 & 9.3 & \textbf{47.0} & \textbf{56.1} & 20.0 \\
			  \rowcolor[HTML]{EFEFEF}
			  CFA w/ cos & 30.3 & 36.6 & 11.3 & 46.9 & 53.2 & 28.2\\\hline
			  A-GEM-DeFRCN & 30.3 & 35.6 & 14.4 & 45.6 & 51.6 & 27.4 \\
			  \rowcolor[HTML]{EFEFEF}
			  CFA-DeFRCN & \textbf{31.4} & 35.5 & \textbf{19.1} & 44.3 & 47.7 & \textbf{34.3}\\
			  
			\bottomrule[1.1pt]
	\end{tabular}}
	\vspace{-0.18cm}
	\caption{Base forgetting comparison between CFA  and A-GEM \cite{agem}. The results are reported for MS-COCO under the 10-shot setting. Compared to A-GEM, CFA shows a better overall performance.}
	\vspace{-0.3cm}
	\label{tab:cl-ablation-study}
\end{table}

==> tables/sota_table_coco.tex <==
\begin{table*}
    \centering
    \begin{tabular}{c | c | c c c | c c c | c c c}
      \Xhline{1pt}
      %%%%%%%%\rule{0pt}{12pt}
    %   \multirow{2}{*}{} &
      \multicolumn{2}{c |}{\multirow{2}{*}{\textbf{Methods} / \textbf{Shots}}} &
      \multicolumn{3}{c |}{\textbf{5 shot}}  &
      \multicolumn{3}{c |}{\textbf{10 shot}}  &
      \multicolumn{3}{c}{\textbf{30 shot}}\\
      %%%%%%%%\rule{0pt}{12pt}
    \multicolumn{2}{c|}{} & \textbf{AP} &  \textbf{bAP} & \textbf{nAP} & \textbf{AP} &  \textbf{bAP} & \textbf{nAP} & \textbf{AP} &  \textbf{bAP} & \textbf{nAP} \\\hline
      %%%%%%%%\rule{0pt}{12pt}
      %=====transfer learning===
      \multirow{5}{*}{\thead{Transfer\\Learning}}
      & FRCN-ft-full\cite{TFA} & 18.0 & 22.0 & 6.0 & 18.1 & 21.0 & 9.2 & 18.6 & 20.6 & 12.5 \\
      & TFA w/ fc\cite{TFA} & 27.5 & 33.9 & 8.4 & 27.9 & 33.9 & 10.0 & 29.7 & 35.1 & 13.4 \\
      & TFA w/ cos\cite{TFA} & 28.1 & 34.7 & 8.3 & 28.7 & 35.0 & 10.0 & 30.3 & 35.8 & 13.7 \\
      & MPSR\cite{MPSR} & - & - & - & 15.3 & 17.1 & 9.7 & 17.1 & 18.1 & 14.1 \\
      & DeFRCN\cite{defrcn} & 28.7 & 33.1 & \second{15.3} & 30.5 & 34.6 & \second{18.5} & 31.6 & 34.7 & \second{22.4}\\\hline
      %%%%%%%%\rule{0pt}{12pt}
      %=====meta learning===
      \multirow{4}{*}{\thead{Meta\\Learning}} & ONCE~\cite{ONCE} & 13.7 & 17.9 & 1.0 & 13.7 & 17.9 & 1.2 & - & - & -  \\
      %%%%%%%%\rule{0pt}{12pt}
       & Meta R-CNN$^{*}$\cite{MetaRCNN} & 3.6 & 3.5 & 3.8 & 5.4 & 5.2 & 6.1 & 7.8 & 7.1 & 9.9 \\
       & FSRW\cite{FSRW} & - & - & - & - & - & 5.6 & - & - & 9.1 \\
       & FsDetView$^{*}$\cite{FsDetView} & 5.9 & 5.7 & 6.6 & 6.7 & 6.4 & 7.6 & 10.0 & 9.3 & 12.0 \\\hline
       %%%%%%%%\rule{0pt}{12pt}
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
        % \multirow{3}{*}{Ours}
       & CFA w/ fc & \best{30.1} & \best{37.1} & 9.0 & 30.8 & \best{37.6} & 10.5 & \second{31.9} & \best{37.7} & 14.7\\
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
       Ours & CFA w/ cos & 29.7 & \second{36.3} & 9.8 & 30.3 & \second{36.6} & 11.3 & 31.7 & 37.0 & 15.6 \\
      \rowcolor[HTML]{EFEFEF}
      \cellcolor[HTML]{FFFFFF}
      & CFA-DeFRCN & \best{30.1} & 35.0 & \best{15.6} & \best{31.4} & 35.5 & \best{19.1} & \best{32.0} & 35.0 & \best{23.0} \\
       \hline
       \hline
       & Retentive R-CNN\cite{gfsod} & 31.5 & 39.2 & 8.3 & 32.1 & 39.2 & 10.5 & 32.9 & 39.3 & 13.8 \\
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
       Retentive-RCNN & CFA w/ fc & 26.1 & 32.0 & 8.5 & 26.4 & 31.9 & 9.9 & 27.6 & 32.1 & 13.9\\
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
       Evaluation Protocol & CFA w/ cos & \best{32.0} & \best{39.5} & \best{9.6} & \best{32.4} & \best{39.4} & \best{11.3} & \best{33.4} & \best{39.5} & \best{15.1} \\
        \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
        & CFA-DeFRCN & 23.7 & 26.6 & 15.1 & 24.7 & 26.9 & 18.2 & 0 & 0 & 0 \\
       \Xhline{1pt}
    \end{tabular}
    \caption{G-FSOD experimental results for 5,10,30-shot settings on MS-COCO. We report AP, bAP, nAP for all, base, and novel classes, respectively. Colored results represent the {\color{red}best} and {\color{blue}second-best}. '*' represents results reported in \cite{gfsod} and \cite{defrcn}. '-' denotes unreported results in the original work.}
    \label{tab:coco}
\end{table*}

==> tables/sota_table_coco_multiple_runs_new.tex <==
\begin{table*}
    \centering
    \begin{tabular}{c | c | c c c | c c c | c c c}
      \Xhline{1pt}
      \multirow{2}{*}{\textbf{Methods} / \textbf{Shots}} & \multirow{2}{*}{\textbf{Seed}} &
      \multicolumn{3}{c |}{\textbf{5 shot}}  &
      \multicolumn{3}{c |}{\textbf{10 shot}}  &
      \multicolumn{3}{c}{\textbf{30 shot}}\\
      & & \textbf{AP} &  \textbf{bAP} & \textbf{nAP} & \textbf{AP} &  \textbf{bAP} & \textbf{nAP} & \textbf{AP} &  \textbf{bAP} & \textbf{nAP} \\ \Xhline{1pt}
      TFA w/ fc\cite{TFA} & 0-9 & 25.6 & 31.8 & 6.9 & 26.2 & 32 & 9.1 & 28.4 & 33.8 & 12 \\
      TFA w/ cos\cite{TFA} & 0-9 & 25.9 & 32.3 & 7 & 26.6 & 32.4 & 9.1 & 28.7 & 34.2 & 12.1 \\
      DeFRCN\cite{defrcn} & 0-9 & 27.8 & 32.6 & 13.6 & 29.7 & 34.0 & 16.8 & 31.4 & 34.8 & 21.2\\
      \Xhline{1pt}
      CFA w/ fc & 0-9 & - & - & - & - & - & - & - & -& -\\
      \hline
      CFA w/ cos& 0-9 & - & - & - & - & - & - & - & - & - \\
      \hline
      CFA-DeFRCN& 0-9 & - & -& - & - &- & - & - & - & - \\
      \Xhline{1pt}
    \end{tabular}
    \caption{G-FSOD experimental results for 5,10,30-shot settings on MS-COCO. We report AP, bAP, nAP for all, base, and novel classes, respectively. w/E denotes whether the ensemble-learning based evaluation protocol of Retentive-RCNN \cite{gfsod} was used. Colored results represent the {\color{red}best} and {\color{blue}second-best}. '*' represents results reported in \cite{gfsod} and \cite{defrcn}. '-' denotes unreported results in the original work.}
    \label{tab:coco}
\end{table*}

==> tables/sota_table_coco_novel.tex <==
\begin{table}[h!]
%\vspace*{-2.5mm}
\begin{center}
\centering
\setlength{\tabcolsep}{2.486pt}
\resizebox{0.474\textwidth}{!}{
\begin{tabular}[t]{ c | l | ccc }
\toprule[1.0pt]

Shot & Method & AP & AP50 & AP75  \\

\midrule[0.68pt]

\multirow{5}{*}{5} & FRCN-ft-full\;\cite{FasterR-CNN}\,$\ddag$\,$\S$ & 4.6 & 8.7 & 4.4 \\
& TFA w/ cos\;\cite{TFA}\,$\ddag$\,$\S$ & 7.0 & 13.3 & 6.5 \\
& FsDetView\;\cite{FsDetView}\,$\S$ & 10.7 & 24.5 & 6.7 \\
& Deformable-DETR-ft-full\,\cite{DETR}\,$\S$ & 7.4 & 12.3 & 7.7 \\
& DeFRCN\;\cite{defrcn}\, & 15.5 & 29.4 & 14.2 \\
& Meta-DETR\;\cite{MetaDetR}\,$\S$ & 15.4 & 25.0 & \textbf{15.8} \\
& \cellcolor{black!6}CFA-DeFRCN (Ours)\,$\S$ & \cellcolor{black!6}\textbf{15.6} & \cellcolor{black!6}\textbf{29.1} & \cellcolor{black!6}15.2 \\
\midrule[0.68pt]

\multirow{14}{*}{10} & FRCN-ft-full\;\cite{FasterR-CNN}\,$\ddag$\,$\S$ & 5.5 & 10.0 & 5.5 \\
& Meta-YOLO\;\cite{FSRW} & 5.6 & 12.3 & 4.6 \\
& Meta R-CNN\;\cite{MetaRCNN} & 8.7 & 19.1 & 6.6 \\
& TFA w/ cos\;\cite{TFA}\,$\ddag$\,$\S$ & 9.1 & 17.1 & 8.8 \\
& Meta\,Det\;\cite{MetaDet} & 7.1 & 14.6 & 6.1 \\
& FSOD\;\cite{FSOD-RPN} & 12.0 & 22.4 & 11.8 \\
& FsDetView\;\cite{FsDetView}\,$\S$ & 12.5 & 27.3 & 9.8 \\
& MPSR\;\cite{MPSR}\,$\ddag$ & 9.8 & 17.9 & 9.7  \\
& FSCE\;\cite{FSCE}\,$\ddag$\,$\S$ & 11.1 & - & 9.8 \\
& CME\;\cite{CME}\,$\ddag$ & 15.1 & 24.6 & 16.4 \\
& Deformable-DETR-ft-full\,\cite{DETR}\,$\S$ & 11.7 & 19.6 & 12.1 \\
& DeFRCN\;\cite{defrcn} & 18.3 & 33.7 & 17.4 \\
& Meta-DETR\;\cite{MetaDetR}\,$\ddag$\,$\S$ & 19.0 & 30.5 & \textbf{19.7} \\

& \cellcolor{black!6}CFA-DeFRCN (Ours)\,$\S$ & \cellcolor{black!6}\textbf{19.1} & \cellcolor{black!6}\textbf{34.8} & \cellcolor{black!6}18.7\\

\midrule[0.66pt]

\multirow{13}{*}{30} & FRCN-ft-full\;\cite{FasterR-CNN}\,$\ddag$\,$\S$ & 7.4 & 13.1 & 7.4 \\

& Meta-YOLO\;\cite{FSRW} & 9.1 & 19.0 & 7.6\\

& Meta R-CNN\;\cite{MetaRCNN} & 12.4 & 25.3 & 10.8 \\

& TFA w/ cos\;\cite{TFA}\,$\ddag$\,$\S$ & 12.1 & 22.0 & 12.0 \\

& Meta\,Det\;\cite{MetaDet} & 11.3 & 21.7 & 8.1\\

& FsDetView\;\cite{FsDetView}\,$\S$ & 14.7 & 30.6 & 12.2 \\

& MPSR\;\cite{MPSR}\,$\ddag$\ & 14.1 & 25.4 & 14.2 \\

& FSCE\;\cite{FSCE}\,$\ddag$\,$\S$ & 15.3 & - & 14.2 \\

& CME\;\cite{CME}\,$\ddag$ & 16.9 & 28.0 & 17.8 \\

& Deformable-DETR-ft-full\,\cite{DETR}\,$\S$ & 16.3 & 27.2 & 16.7 \\

& DeFRCN\;\cite{defrcn}\ & 22.6 & 39.8 & 22.8 \\



& Meta-DETR\;\cite{MetaDetR}\,$\ddag$\,$\S$ & 22.2 & 35.0 & 22.8 \\

& \cellcolor{black!6}CFA-DeFRCN (Ours)\,$\S$ & \cellcolor{black!6}\textbf{23.0} & \cellcolor{black!6}\textbf{40.5} & \cellcolor{black!6}\textbf{23.0} \\

\bottomrule[1.0pt]

\end{tabular}
}
\end{center}
\vspace*{-3.0mm}
\caption{Few-shot detection performance on MS-COCO for the novel categories.  $\ddag$ indicates methods using multi-scale features. $\S$ indicates results averaged on multiple runs.}
\label{tab:coco_novel}
\vspace*{-2.0mm}
\end{table}

==> tables/sota_table_voc_novel.tex <==
\begin{table*}
\footnotesize
    \centering
    \begin{tabular}{p{0.9cm}| c | c c c c c | c c c c c | c c c c c}
      \Xhline{1pt}
      %%%%%%%%\rule{0pt}{12pt}
    %   \multirow{2}{*}{} &
      \multicolumn{2}{c |}{\multirow{2}{*}{\textbf{Methods} / \textbf{Shots}}} &
      \multicolumn{5}{c |}{\textbf{Novel Set 1}}  &
      \multicolumn{5}{c |}{\textbf{Novel Set 2}}  &
      \multicolumn{5}{c}{\textbf{Novel Set 3}}\\
      %%%%%%%%\rule{0pt}{12pt}
    \multicolumn{2}{c |}{} & 1 &  {2} & {3} & {5} &  {10} & 1 &  {2} & {3} & {5} &  {10} & 1 &  {2} & {3} & {5} &  {10} \\\hline
      %%%%%%%%\rule{0pt}{12pt}
      %=====transfer learning===
      \multirow{6}{*}{\thead{Transfer\\Learning}}
      & FRCN-ft-full\cite{TFA} & 15.2 & 20.3 & 29.0 & 25.5 & 28.7 & 13.4 & 20.6 & 28.6 & 32.4 & 38.8 & 19.6 & 20.8 & 28.7 & 42.2 & 42.1 \\
      %& FRCN-BCE & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\\cline{2-{17}}
      & TFA w/ fc\cite{TFA} & 36.8 & 29.1 & 43.6 & 55.7 & 57.0 & 18.2 & 29.0 & 33.4 & 35.5 & 39.0 & 27.7 & 33.6 & 42.5 & 48.7 & 50.2 \\
      & TFA w/ cos\cite{TFA} & 39.8 & 36.1 & 44.7 & 55.7 & 56.0 & 23.5 & 26.9 & 34.1 & 35.1 & 39.1 & 30.8 & 34.8 & 42.8 & 49.5 & 49.8 \\
      & MPSR\cite{MPSR} & 42.8 & 43.6 & 48.4 & 55.3 & 61.2 & 29.8 & 28.1 & 41.6 & 43.2 & 47.0 & 35.9 & 40.0 & 43.7 & 48.9 & 51.3 \\
      & Retentive R-CNN\cite{gfsod}& 42.4 & 45.8 & 45.9 & 53.7 & 56.1 & 21.7 & 27.8 & 35.2 & 37.0 & 40.3 & 30.2 & 37.6 & 43.0 & 49.7 & 50.1 \\
    & DeFRCN\cite{defrcn} & \second{57.0} & \second{58.6} & \second{64.3} & \second{67.8} & \second{67.0} &
    \second{35.8} & \second{42.7} & \second{51.0} & \second{54.4} & \second{52.9} & \second{52.5} & \second{56.5} & \second{55.8} & \second{60.7} & \best{62.5} \\\hline
      %%%%%%%%\rule{0pt}{12pt}
      %=====meta learning===
      \multirow{4}{*}{\thead{Meta\\Learning}} &
      %%%%%%%%\rule{0pt}{12pt}
      Meta R-CNN$^{*}$\cite{MetaRCNN} & 16.8 & 20.1 & 20.3 & 38.2 & 43.7 & 7.7 & 12.0 & 14.9 & 21.9 & 31.1 & 9.2 & 13.9 & 26.2 & 29.2 & 36.2 \\
       & FSRW\cite{FSRW} & 14.8 & 15.5 & 26.7 & 33.9 & 47.2 & 15.7 & 15.3 & 22.7 & 30.1 & 39.2 & 19.2 & 21.7 & 25.7 & 40.6 & 41.3 \\
       & MetaDet\cite{MetaDet} & 18.9 & 20.6 & 30.2 & 36.8 & 49.6 & 21.8 & 23.1 & 27.8 & 31.7 & 43.0 & 20.6 & 23.9 & 29.4 & 43.9 & 44.1\\
       & FsDetView$^*$\cite{FsDetView} & 25.4 & 20.4 & 37.4 & 36.1 & 42.3 & 22.9 & 21.7 & 22.6 & 25.6 & 29.2 & 32.4 & 19.0 & 29.8 & 33.2 & 39.8 \\\hline
       %%%%%%%%\rule{0pt}{12pt}
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
       & CFA w/ fc & 42.6 & 38.3 & 46.7 & 53.6 & 54.3 & 18.0 & 25.6 & 34.2 & 33.5 & 38.2 & 32.7 & 35.4 & 40.0 & 45.9 & 48.8 \\
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
       Ours & CFA w/ cos & 44.7 & 41.7 & 45.5 & 51.0 & 51.4 & 18.7 & 23.9 & 32.6 & 32.5 & 0 & 31.7 & 32.8 & 39.1 & 43.7 & 46.7 \\
        \rowcolor[HTML]{EFEFEF}
        \cellcolor[HTML]{FFFFFF}
        & CFA-DeFRCN & \best{58.8} & \best{63.3} & \best{65.2} & \best{68.4} & \best{67.2} & \best{37.3} & \best{45.2} & \best{51.9} & \best{54.5} & \best{53.2} & \best{55.1} & \best{57.8} & \best{56.4} & \best{60.8} & \second{62.4} \\
        \Xhline{1pt}
    \end{tabular}
    \caption{G-FSOD experimental results for 1,2,3,5,10-shot settings on the three novel sets of Pascal VOC (nAP50). Colored results represent the {\color{red}best} and {\color{blue}second-best}. '*' represents results reported in \cite{gfsod} and \cite{defrcn}. We achieve state-of-the-art novel performance (nAP50) across the three different splits under different few-shot settings.}
    \label{tab:voc-novel}
\end{table*}

==> tables/sota_table_voc_novel_multiple_runs.tex <==
\begin{table*}
\footnotesize
    \centering
    \begin{tabular}{c| c | c c c c c }
      \Xhline{1pt}
      \multirow{2}{*}{\textbf{Set}} &
      \multirow{2}{*}{\textbf{Methods}} &
      \multicolumn{5}{c}{\textbf{Shots}}  &
       & & 1 &  {2} & {3} & {5} &  {10} \\ \Xhline{1pt}
      & CFA w/ fc& 28.2$\pm$3.1 & 35.0$\pm$1.9 & 41.9$\pm$1.4 & 47.8$\pm$1.6 & 53.3$\pm$1.6 \\
      & CFA w/ cos& 30.9$\pm$3.9 & 40.9$\pm$2.5 & 47.8$\pm$2.4 & 53.1$\pm$1.4 & 56.1$\pm$1.4 \\
      & DeFRCN\cite{defrcn} & 43.8$\pm$4.3 & 57.5$\pm$2.5 & 61.4$\pm$1.7 & 65.3$\pm$0.9 & 67.0$\pm$1.4 \\
      \multirow{-4}{*}{\textbf{Novel Set 1}} & CFA-DeFRCN & 45.4$\pm$4.9 & 60.3$\pm$2.2 & 62.1$\pm$1.4 & 66.4$\pm$0.9 & 67.6$\pm$1.2 \\
       \hline
       & CFA w/ fc & 20.0$\pm$3.5 & 26.4$\pm$2.9 & 32.8$\pm$2.2 & 37.3$\pm$1.7 & 41.8$\pm$1.9 \\
       & CFA w/ cos & 21.0$\pm$3.5 & 29.0$\pm$2.3 & 34.6$\pm$2.3 & 38.9$\pm$1.2 & 43.0$\pm$1.9 \\
       & DeFRCN\cite{defrcn} & 31.5$\pm$3.6 & 40.9$\pm$2.2 & 45.6$\pm$2.0 & 50.1$\pm$1.4 & 52.9$\pm$1.1 \\ 
       \multirow{-4}{*}{\textbf{Novel Set 2}} & CFA-DeFRCN & 32.9$\pm$3.7 & 42.3$\pm$2.2 & 47.1$\pm$1.9 & 51.2$\pm$1.4 & 55.3$\pm$1.3 \\ 
       \hline
       & CFA w/ fc & 20.3$\pm$3.4 & 26.4$\pm$3.1 & 34.3$\pm$2.5 & 41.2$\pm$2.4 & 46.5$\pm$1.6 \\
       & CFA w/ cos & 21.5$\pm$4.7 & 30.4$\pm$4.1 & 38.4$\pm$2.8 & 45.5$\pm$2.1 & 49.9$\pm$1.0 \\
       & DeFRCN\cite{defrcn} & 38.2$\pm$6.8 & 50.9$\pm$2.8 & 54.1$\pm$2.2 & 59.2$\pm$1.2 & 61.9$\pm$1.3 \\
       \multirow{-4}{*}{\textbf{Novel Set 3}} & CFA-DeFRCN & 41.4$\pm$5.8 & 52.9$\pm$3.0 & 56.1$\pm$1.7 & 60.3$\pm$1.1 & 62.9$\pm$0.9 \\
       \hline
    \end{tabular}
    \caption{G-FSOD experimental results for 1,2,3,5,10-shot settings on the three novel sets of Pascal VOC (nAP50).}
    \label{tab:voc-novel}
\end{table*}

==> tables/sota_table_voc_overall.tex <==
\begin{table*}
\footnotesize
    \centering
    \begin{tabular}{p{0.9cm}| c | c c c c c | c c c c c | c c c c c}
      \Xhline{1pt}
      %%%%%%%%\rule{0pt}{12pt}
    %   \multirow{2}{*}{} &
      \multicolumn{2}{c |}{\multirow{2}{*}{\textbf{Methods} / \textbf{Shots}}} &
      \multicolumn{5}{c |}{\textbf{All Set 1}}  &
      \multicolumn{5}{c |}{\textbf{All Set 2}}  &
      \multicolumn{5}{c}{\textbf{All Set 3}}\\
      %%%%%%%%\rule{0pt}{12pt}
    \multicolumn{2}{c |}{} & 1 &  {2} & {3} & {5} &  {10} & 1 &  {2} & {3} & {5} &  {10} & 1 &  {2} & {3} & {5} &  {10} \\\hline
      %=====transfer learning===
      \multirow{5}{*}{\thead{Transfer\\Learning}} 
      & FRCN-ft-full\cite{TFA} & 55.4 & 57.1 & 56.8 & 60.1 & 60.9 & 50.1 & 53.7 & 53.6 & 55.9 & 55.5 & 58.5 & 59.1 & 58.7 & 61.8 & 60.8 \\
      %& FRCN-BCE & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\\cline{2-{17}}
      & TFA w/ fc\cite{TFA} & 69.3 & 66.9 & 70.3 & 73.4 & 73.2 & 64.7 & 66.3 & 67.7 & 68.3 & 68.7 & 67.8 & 68.9 & 70.8 & 72.3 & 72.2 \\
      & TFA w/ cos\cite{TFA} & 69.7 & 68.2 & 70.5 & 73.4 & 72.8 & 65.5 & 65.0 & 67.7 & 68.0 & 68.6 & 67.9 & 68.6 & 71.0 & 72.5 & 72.4 \\
      & MPSR\cite{MPSR} & 56.8 & 60.4 & 62.8 & 66.1 & 69.0 &
        53.1 & 57.6 & 62.8 & 64.2 & 66.3 & 55.2 & 59.8 & 62.7 & 66.9 & 67.7 \\
        & Retentive R-CNN\cite{gfsod} & 71.3 & 72.3 & 72.1 & 74.0 & \second{74.6} & 66.8 & 68.4 & 70.2 & \second{70.7} & \second{71.5} & 69.0 & 70.9 & 72.3 & 73.9 & \best{74.1} \\
      & DeFRCN\cite{defrcn} & \second{73.0} & \second{73.2} & \second{73.7} & \second{75.1} & 74.4 &
        \second{68.6} & \second{69.8} & \second{71.0} & \best{72.5} & \second{71.5} & \second{72.5} & \second{73.5} & \second{72.7} & \second{74.1} & 73.9 \\\hline
      %%%%%%%%\rule{0pt}{12pt}
      %=====meta learning===
      \multirow{3}{*}{\thead{Meta\\Learning}} &
      %%%%%%%%\rule{0pt}{12pt}
        Meta R-CNN$^{*}$\cite{MetaRCNN} & 17.5 & 30.5 & 36.2 & 49.3 & 55.6 & 19.4 & 33.2 & 34.8 & 44.4 & 53.9 & 20.3 & 31.0 & 41.2 & 48.0 & 55.1 \\
       & FSRW\cite{FSRW} & 53.5 & 50.2 & 55.3 & 56.0 & 59.5 & 55.1 & 54.2 & 55.2 & 57.5 & 58.9 & 54.2 & 53.5 & 54.7 & 58.6 & 57.6 \\
       & FsDetView$^*$\cite{FsDetView} & 36.4 & 40.3 & 40.1 & 50.0 & 55.3 & 36.3 & 43.7 & 41.6 & 45.8 & 54.1 & 37.0 & 39.5 & 40.7 & 50.7 & 54.8 \\\hline
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
       & CFA w/ fc & 70.1 & 68.7 & 71.4 & 72.6 & 72.7 & 65.2 & 66.5 & 68.7 & 68.7 & 69.8 & 68.3 & 68.1 & 70.3 & 71.5 & 71.6 \\
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
       Ours & CFA w/ cos & 70.2 & 68.8 & 70.2 & 71.7 & 71.8 & 63.7 & 65.2 & 67.4 & 67.7 & 0 & 67.2 & 66.5 & 70.2 & 70.3 & 71.0 \\
       \rowcolor[HTML]{EFEFEF}
       \cellcolor[HTML]{FFFFFF}
       & CFA-DeFRCN & \best{73.5} & \best{74.8} & \best{74.5} & \best{76.0} & \best{74.7} & \best{69.5} & \best{71.4} & \best{72.1} & \best{72.5} & \best{71.7} & \best{73.1} & \best{74.1} & \best{73.5} & \best{74.7} & \second{74.0} \\ \hline
       
       \Xhline{1pt}
    \end{tabular}
    \caption{G-FSOD experimental results for 1,2,3,5,10-shot settings on the three all sets of Pascal VOC (AP50). Colored results represent the {\color{red}best} and {\color{blue}second-best}. '*' represents results reported in \cite{gfsod} and \cite{defrcn}. Across the three different sets, we deliver the best overall performance (AP50) compared to the aforementioned approaches.}
    \label{tab:voc-all}
\end{table*}

==> tables/sota_table_voc_overall_multiple_runs.tex <==
\begin{table*}
\footnotesize
    \centering
    \begin{tabular}{c| c | c c c c c }
      \Xhline{1pt}
      \multirow{2}{*}{\textbf{Set}} &
      \multirow{2}{*}{\textbf{Methods}} &
      \multicolumn{5}{c}{\textbf{Shots}}  &
       & & 1 &  {2} & {3} & {5} &  {10} \\ \Xhline{1pt}
      & CFA w/ fc& 66.3$\pm$0.8 & 68.0$\pm$0.5 & 70.1$\pm$0.4 & 71.7$\pm$0.5 & 73.2$\pm$0.5 \\
      & CFA w/ cos& 66.5$\pm$0.9 & 69.2$\pm$0.6 & 71.1$\pm$0.6 & 72.5$\pm$0.4 & 73.4$\pm$0.4 \\
      & DeFRCN\cite{defrcn} & 67.8$\pm$1.4 & 71.3$\pm$0.8 & 72.6$\pm$0.5 & 73.6$\pm$0.5 & 74.1$\pm$0.5 \\
      \multirow{-4}{*}{\textbf{All Set 1}} & CFA-DeFRCN & 69.0$\pm$1.4 & 72.6$\pm$0.7 & 73.1$\pm$0.4 & 74.0$\pm$0.5 & 74.3$\pm$0.4 \\
       \hline
       & CFA w/ fc & 64.9$\pm$0.9 & 66.4$\pm$0.7 & 68.3$\pm$0.5 & 69.6$\pm$0.3 & 70.8$\pm$0.5 \\
       & CFA w/ cos & 64.1$\pm$0.9 & 66.5$\pm$0.5 & 68.1$\pm$0.5 & 69.3$\pm$0.2 & 70.4$\pm$0.4 \\
       & DeFRCN\cite{defrcn} & 65.2$\pm$1.0 & 68.0$\pm$0.8 & 69.2$\pm$0.6 & 70.6$\pm$0.6 & 71.3$\pm$0.5 \\
       \multirow{-4}{*}{\textbf{All Set 2}} & CFA-DeFRCN & 66.4$\pm$1.0 & 69.0$\pm$0.8 & 70.4$\pm$0.7 & 71.3$\pm$0.7 & 72.1$\pm$0.4 \\ 
       \hline
       & CFA w/ fc & 65.2$\pm$0.8 & 66.8$\pm$0.8 & 69.1$\pm$0.7 & 70.9$\pm$0.6 & 72.3$\pm$0.4 \\
       & CFA w/ cos & 64.9$\pm$1.2 & 67.5$\pm$1.0 & 69.7$\pm$0.8 & 71.6$\pm$0.5 & 72.7$\pm$0.3 \\
       & DeFRCN\cite{defrcn} & 66.9$\pm$2.0 & 70.6$\pm$0.8 & 71.2$\pm$0.6 & 72.9$\pm$0.5 & 73.5$\pm$0.3 \\
       \multirow{-4}{*}{\textbf{All Set 3}} & CFA-DeFRCN & 68.3$\pm$1.6 & 71.4$\pm$0.8 & 72.3$\pm$0.5 & 73.5$\pm$0.5 & 74.0$\pm$0.3 \\
       \hline
    \end{tabular}
    \caption{G-FSOD experimental results for 1,2,3,5,10-shot settings on the three all sets of Pascal VOC (AP50).}
    \label{tab:voc-all}
\end{table*}

==> tables/sota_table_voc_overall_multiple_runs_new.tex <==
\begin{table*}
\footnotesize
    \centering
    \begin{tabular}{c| c | c c c c c | c c c c c | c c c c c}
      \Xhline{1pt}
      \multirow{2}{*}{\textbf{Methods} / \textbf{Shots}} &
      \multirow{2}{*}{\textbf{Seed}} &
      \multicolumn{5}{c |}{\textbf{All Set 1}}  &
      \multicolumn{5}{c |}{\textbf{All Set 2}}  &
      \multicolumn{5}{c}{\textbf{All Set 3}}\\

      & & 1 &  {2} & {3} & {5} &  {10} & 1 &  {2} & {3} & {5} &  {10} & 1 &  {2} & {3} & {5} &  {10} \\ \Xhline{1pt}
       CFA w/ fc& 0 & 69.5 & 68.2 & 69.8 & 73.5 & 74.3 & 66.0 & 66.9 & 69.2 & 70.1 & 71.1 & 67.7 & 69.0 & 70.9 & 72.6 & 73.5 \\
       CFA w/ fc& 1 & 67.6 & 69.5 & 71.0 & 72.1 & 73.5 & 66.2 & 68.0 & 69.5 & 69.9 & 72.1 & 65.2 & 68.2 & 69.7 & 71.4 & 72.8 \\
       CFA w/ fc& 2 & 65.4 & 67.4 & 71.1 & 70.3 & 71.7 & 66.0 & 68.0 & 69.4 & 69.5 & 71.3 & 63.0 & 67.7 & 70.3 & 70.7 & 72.6 \\
       CFA w/ fc& 3 & 66.2 & 68.4 & 69.7 & 71.2 & 73.5 & 64.7 & 66.1 & 68.7 & 69.1 & 70.2 & 65.6 & 66.4 & 69.5 & 70.6 & 72.8 \\
       CFA w/ fc& 4 & 66.2 & 66.8 & 69.8 & 71.8 & 71.8 & 64.3 & 67.3 & 67.9 & 70.1 & 71.0 & 64.9 & 65.0 & 67.2 & 70.4 & 71.8 \\
       CFA w/ fc& 5 & 66.1 & 67.1 & 69.3 & 71.3 & 73.3 & 64.0 & 66.8 & 68.3 & 69.4 & 71.0 & 67.1 & 66.2 & 68.2 & 69.8 & 71.4 \\
       CFA w/ fc& 6 & 65.0 & 67.8 & 69.7 & 71.4 & 73.9 & 66.4 & 66.1 & 67.3 & 68.5 & 70.3 & 65.5 & 67.4 & 69.1 & 71.3 & 72.1 \\
       CFA w/ fc& 7 & 65.1 & 67.7 & 70.0 & 71.1 & 73.8 & 61.4 & 64.6 & 67.9 & 69.8 & 70.5 & 64.4 & 66.5 & 68.2 & 69.5 & 71.9 \\
       CFA w/ fc& 8 & 66.8 & 68.8 & 70.8 & 71.6 & 72.6 & 66.0 & 64.8 & 66.7 & 68.9 & 69.2 & 64.7 & 66.1 & 68.2 & 70.1 & 72.7 \\
       CFA w/ fc& 9 & 65.3 & 68.0 & 69.7 & 72.4 & 73.3 & 63.9 & 65.9 & 68.3 & 70.3 & 71.2 & 63.7 & 19.9 & 69.8 & 72.1 & 71.6 \\
       CFA w/ fc& 0-9 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
       \hline
       CFA w/ cos& 0  & 69.1 & 69.8 & 71.9 & 73.6 & 73.9 & 64.8 & 66.5 & 68.3 & 69.5 & 70.5 & 67.7 & 69.7 & 71.9 & 73.0 & 73.5 \\
       CFA w/ cos& 0-9  & 66.5$\pm$0.9 & 69.2$\pm$0.6 & 71.1$\pm$0.6 & 72.5$\pm$0.4 & 73.3$\pm$0.4 & 64.1$\pm$0.9 & 66.5$\pm$0.5 & 68.1$\pm$0.5 & 69.3$\pm$0.2 & 70.4$\pm$0.4 & 64.9$\pm$1.2 & 67.5$\pm$1.0 & 69.7$\pm$0.8 & 71.6$\pm$0.5 & 72.7$\pm$0.3 \\
       \hline
       CFA-DeFRCN& 0 & 73.8 & 74.6 & 74.5 & 76.0 & 74.4 & 69.3 & 71.4 & 72.0 & 73.3 & 72.0 & 72.9 & 73.9 & 73.0 & 74.1 & 74.6 \\
       CFA-DeFRCN& 1 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 2 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 3 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 4 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 5 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 6 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 7 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 8 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 9 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
       CFA-DeFRCN& 0-9 & - & - & - & - & - & - & - & - & - & - & - & - & - & - &- \\
        \Xhline{1pt}
    \end{tabular}
    \caption{G-FSOD experimental results for 1,2,3,5,10-shot settings on the three all sets of Pascal VOC (AP50). w/E denotes whether the ensemble-learning based evaluation protocol of Retentive-RCNN \cite{gfsod} was used. Colored results represent the {\color{red}best} and {\color{blue}second-best}. '*' represents results reported in \cite{gfsod} and \cite{defrcn}.}
    \label{tab:voc-all}
    \vspace{-2em}
\end{table*}
